Dual-Space Augmented Intrinsic-LoRA for Wind Turbine Segmentation

Accurate segmentation of wind turbine blade (WTB) images is critical for effective assessments, as it directly influences the performance of automated damage detection systems. Despite advancements in large universal vision models, these models often underperform in domain-specific tasks like WTB segmentation. To address this, we extend Intrinsic LoRA for image segmentation, and propose a novel dual-space augmentation strategy that integrates both image-level and latent-space augmentations. The image-space augmentation is achieved through linear interpolation between image pairs, while the latent-space augmentation is accomplished by introducing a noise-based latent probabilistic model. Our approach significantly boosts segmentation accuracy, surpassing current state-of-the-art methods in WTB image segmentation.

==> Chapters/OldIntroduction.tex <==
Image segmentation of complex real-world structures has always been a core problem in field of computer vision. It has applications in various fields such as medical imaging, robot vision, and industrial maintenance. Deep learning methods, particularly convolutional neural networks (CNNs) have been at the forefront of image segmentation research. Encoder-Decoder architectures~\cite{deeplab, sw} have become a fundamental framework offering an effective approach towards capturing and reconstructing spatial relationships. Earlier methods like DeepLabv3+ \cite{deeplabv3+} and ResNeSt \cite{resnest} have also utilized CNNs and post-processing methods to enhance their respective segmentation maps. The attention mechanism has also been introduced to this architecture in several studies \cite{attention2, bmvc}. One of the key examples, however, is the U-Net \cite{unet}, a powerful framework involving skip connections from the encoder to the decoder, that has inspired numerous subsequent models for a diverse range of tasks. A hybrid approach UNetFormer \cite{unetformer} achieved good results which constituted of a CNN-based encoder and a transformer-based decoder. Earlier research on turbine segmentation such as BU-Net \cite{bunet} focused on using a custom U-Net aided by a post-processing hole-filling algorithm to create a robust framework. 

For particular downstream tasks, having a comprehensive and extensive dataset is not always possible. Recent studies have utilized self-supervised learning and generative models for image segmentation. Meta's DINO \cite{dino} presented that self-supervised vision transformers (ViT) automatically learn explicit information about the data which allows extraction of segmentation maps from the self-attention maps. Intrinsic LoRA \cite{intrinsic-lora} further proves that generative models like GANs, Autoregressive models, and Diffusion models like Stable Diffusion \cite{stable-diffusion} implicitly learn image intrinsics. They utilized Low-Rand Adaptation (LoRA) \cite{lora} to fine-tune several generative models with weak supervision from ground-truth depth and surface normal maps. We believe this method can be extended to extract segmentation maps for our turbine detection problem.

Several augmentation methods have been used to enhance baseline model performance. Predominantly, we can see flipping, rotation and cropping. Mixup \cite{mixup}, an image space augmentation method has proven to be quite effective. Some studies have presented that injection of noise \cite{Sønderby2016a, jenni2019stabilizing} has also helped stabilize training generative models. However, there is missing space which we believe is augmentation in the latent space. While Stable Diffusion does explore the diffusion process in latent space we would like to understand how noise injection in latent space would affect generative models. We propose an adaptation of Intrinsic LoRA to image segmentation and present improvements in baseline metrics by injecting latent noise. We also present dual-space augmentation where we combine Mixup with our latent noise. As a result, we obtain a robust model that achieves state-of-the-art results on our turbine dataset.

\begin{figure}[t!]
%\begin{minipage}[b]{0.94\linewidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/fig1new.png}
  \vspace{-0.3cm}
%\end{minipage}
\caption{\textbf{General schema of Segmentation-based Intrinsic LoRA (SI-LoRA) with dual-space augmentation.} }
%The training mechanism is similar to Intrinsic LoRA \cite{intrinsic-lora}. Instead of intrinsics, we supervise the training process with few segmentation maps. Augmentations in image and latent space are added.
\label{fig:basic_pipeline}
\vspace{-0.55cm}
\end{figure}


==> Chapters/OldMethods.tex <==
\subsection{Intrinsic LoRA}

This study explores the findings in Intrinsic-LoRA \cite{intrinsic-lora} demonstrating the implicit understanding of image intrinsics in generative diffusion models. An image-to-image generative diffusion model can be supervised with a few labeled samples to generate desired intrinsics by introducing some learnable LoRA adaptors $\boldsymbol{\theta}$. In the case of Stable Diffusion~\cite{stable-diffusion}, it is successfully done by using these adaptors on top of the self and cross-attention layers~\cite{attention} of the U-Net model~\cite{unet}. For generating depth maps $\mathbf{y}^{(H \times W \times 3)}$ from an image $\mathbf{x}^{(H \times W \times 3)}$, the objective function to train the LoRA adaptors~\cite{lora} is defined as:
%d is a dissimilarity metric
\begin{equation} \label{eq:i-lora}
 \min_{\boldsymbol{\theta}} \mathbb{E}_{\mathbf{x}} [d(U_{\boldsymbol{\theta}} (\mathbf{z}_{E}, T(t)), E(\mathbf{y}))]  ~,
\end{equation}
where $E$ is the Stable Diffusion's Encoder, and $U_{\boldsymbol{\theta}}$ is the denoising U-Net model, which is actually a single step dense predictor in the case of Intrinsic LoRA. $d$ is a dissimilarity metric which depends on the image intrinsic to be extracted. As shown in Figure~\ref{fig:introd}, for an input image $\mathbf{x}$ in the RGB space, the Encoder $E$ compresses it to a lower-dimensional latent space. 
\begin{equation} \label{eq:Encoder}
    \mathbf{z}_{E} = E(\mathbf{x}) ~.
\end{equation}

The obtained latent vector $\mathbf{z}_{E}$ is fed to the U-Net model. Along with that, the final piece is the text prompt, which in case of Intrinsic LoRA is the image intrinsic to be extracted like "depth", "normal" and so forth. The prompt $t$ is encoded by a pretrained CLIP Tokenizer T \cite{clip}.
\begin{equation} \label{eq:U-Net}
    \mathbf{z}_{U} = U_{\boldsymbol{\theta}} (\mathbf{z}_{E}, T(t)) ~.
\end{equation}

The output latent vector $z_{U}$ is compared with the encoded ground-truth $z_{U|I}$ or $E(y)$. The Decoder $D$ projects the predicted latent vector $z_{U}$ back to the image space, reconstructing the image in the process. It should be noted that both the encoder $E$ and decoder $D$ are frozen during the training.
\begin{equation}
    \hat{\mathbf{y}} = D(\mathbf{z}_U) ~,
\end{equation}
where $\hat{\mathbf{y}}$ is the predicted intrinsic map.

\subsection{Segmentation-based Intrinsic LoRA} \label{sec:si-lora}
Stable Diffusion's variational autoencoder expects a 3-channel output, however, binary masks are single-channel where each pixel is either background or foreground. 
For an image $\mathbf{x}^{(H \times W \times 3)}$ and its corresponding ground-truth segmentation map $\mathbf{m}^{(H \times W)}$.

For compatibility we repeat the single channel mask 3 times and stack it along the channel dimension to effectively create a 3-channel input. The decoded output from the autoencoder is a 3-channel image, which is then converted to a single channel mask by taking the mean across the channel axis. Since the loss in the original method is calculated between the latent encodings, we take $d$ as the Mean Squared Error (MSE) loss. Therefore, the objective function of Eq.~\ref{eq:i-lora} for our problem becomes :
\begin{equation} \label{eq: New Obj Fn}
\min_{\boldsymbol{\theta}} \mathbb{E}_x [MSE(U_{\boldsymbol{\theta}} \circ E(\mathbf{x}), \mathbf{E(y)})] , \quad \hat{\mathbf{m}} = \frac{1}{3}\sum_{c=1}^3 \hat{\textbf{y}}_c ~.
\end{equation}

The text prompt chosen for the segmentation adaptation was- "segmentation map".



\subsection{Dual-Space Data Augmentation} \label{sec:aug}

Having successfully adapted the Intrinsic-LoRA method to our segmentation task, we then focused on improving its performance. Data augmentation in the image space has been extensively studied and implemented to improve on baseline approaches. One remarkable technique is MixUp~\cite{mixup}, which generates artificial images by linear interpolation of multiple images. Specifically, given a pair of images and their corresponding labels from the training set, \((\mathbf{x}_i, \mathbf{m}_i)\) and \((\mathbf{x}_j, \mathbf{m}_j)\), MixUp creates a new augmented sample \((\mathbf{x}', \mathbf{m}')\) as follows:



\begin{equation}
    \mathbf{x}' = \lambda \mathbf{x}_i + (1-\lambda) \mathbf{x}_j ~, \quad
    \mathbf{m}' = \lambda \mathbf{m}_i + (1-\lambda) \mathbf{m}_j ~,
\end{equation}
where \(\lambda \in [0,1]\) is a mixing coefficient sampled from a Beta distribution with parameters $\alpha, \beta = 0.4$, which governs the interpolation between the two images and their labels.

While these techniques have proven effective, our contribution lies in extending augmentation to the latent space. Traditional diffusion models operated in the image space, however, Stable Diffusion~\cite{stable-diffusion} demonstrated the effectiveness of shifting the diffusion process to the latent space. Drawing inspiration from this, we augment the training by injecting noise into the latent encodings $\mathbf{z}_E$. This allows us to maintain the integrity of the maps at the high-dimension and forces the model to map from a bigger latent space. The latent vector for an input image $\mathbf{x}$ which acts as input to $U_{\boldsymbol{\theta}}$ is treated as a Bayesian estimation through an isotropic multivariate Gaussian with an identity covariance matrix:

\begin{equation} \label{eq:gaussian_noise}
  \mathbf{z}_{E} \sim   \mathcal{N}\big( E (\mathbf{x}), \mathbf{Id}  \big) 
\end{equation}


%Eq. \ref{eq:gaussian_noise}
While training Stable Diffusion, the latent space is always scaled to unit variance. Given the latent encoding of an input image is normalized, we introduce further randomness by sampling a noise vector $\epsilon$ from a standard Gaussian distribution. 
Therefore, the algebraic injection of noise is carried out and the input of the U-Net changes to:

\begin{equation}
\mathbf{z}_{E}' = E (\mathbf{x}) + \boldsymbol{\epsilon} , \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0,1) ~.
\end{equation}

Consequently, the augmented latent vector is fed to the U-Net and the Eq \ref{eq:U-Net} becomes:
\begin{equation} \label{eq:prefinal}
    \mathbf{z}_{U}' = U_{\boldsymbol{\theta}}(\mathbf{z}_{E}', T(t)) ~.
\end{equation}

To summarize, after implementing our dual-space augmentation, the Eq.~\ref{eq:prefinal} can now be described as:

\begin{equation}
\mathbf{z}_{U} = U_{\boldsymbol{\theta}} \left( E(\mathbf{\lambda \mathbf{x}_i + (1-\lambda) \mathbf{x}_j}) + \epsilon, T(t) \right)      
\end{equation}

%%% E encoder, D decoder, U U-Net
%%% G = U o E




